Prior-Guided Adversarial Initialization for Fast Adversarial Training

Fast adversarial training (FAT) effectively improves the efficiency of standard adversarial training (SAT). However, initial FAT encounters catastrophic overfitting, i.e.,the robust accuracy against adversarial attacks suddenly and dramatically decreases. Though several FAT variants spare no effort to prevent overfitting, they sacrifice much calculation cost. In this paper, we explore the difference between the training processes of SAT and FAT and observe that the attack success rate of adversarial examples (AEs) of FAT gets worse gradually in the late training stage, resulting in overfitting. The AEs are generated by the fast gradient sign method (FGSM) with a zero or random initialization. Based on the observation, we propose a prior-guided FGSM initialization method to avoid overfitting after investigating several initialization strategies, improving the quality of the AEs during the whole training process. The initialization is formed by leveraging historically generated AEs without additional calculation cost. We further provide a theoretical analysis for the proposed initialization method. We also propose a simple yet effective regularizer based on the prior-guided initialization,i.e., the currently generated perturbation should not deviate too much from the prior-guided initialization. The regularizer adopts both historical and current adversarial perturbations to guide the model learning. Evaluations on four datasets demonstrate that the proposed method can prevent catastrophic overfitting and outperform state-of-the-art FAT methods. The code is released at https://github.com/jiaxiaojunQAQ/FGSM-PGI.

==> algo/FGSM_FIAL.tex <==
\begin{algorithm}[t]
\caption{FGSM-MEPAL}
\label{alg:FGSM_FIAL}
\begin{algorithmic}[1]
\REQUIRE
The epoch $N$, the maximal perturbation $\epsilon$, the maximal label perturbation $\epsilon_{\mathbf{y}}$, the step size $\alpha$, the dataset $\mathcal{D}$ including the benign sample $\mathbf{x}$ and the label $\mathbf{y}$, the dataset size $M$, the network $f(\cdot, \mathbf{w})$ with parameters $\mathbf{w}$, the decay factor $\mu$, the free initialization set $\mathcal{D}^{\mathbf{\boldsymbol{\delta}}}$ and the historical model gradient $\mathcal{D}^{m}$.
%The watermark image $W$, the host image $H$, the well-trained classifier $f$

\FOR{$n=1,...,N$}
\FOR{$i=1,...,M$}
\IF{$n==1$}
\STATE $\boldsymbol{\eta} =\mathbf{U}(-\epsilon ,\epsilon) $
\STATE $\mathbf{g}_{c} =\operatorname{sign}\left(\nabla_{\mathbf{x}_i} \mathcal{L}(f(\mathbf{x}_i+\mathbf{\boldsymbol{\eta}} ; \mathbf{w}), \mathbf{y}_{i})\right)$
\STATE $\mathcal{D}^{m}_{i}= \mathbf{g}_{c}$
\STATE $ \mathbf{\boldsymbol{\delta}} =\Pi_{[-\epsilon, \epsilon]} [ \mathbf{\boldsymbol{\eta}}+ \alpha \cdot \mathbf{g}_{c} ]$
\STATE $\mathbf{y}_{i}=\textrm{norm}(\mathbf{y}_{i}+\mathbf{\boldsymbol{\eta}}_{\mathbf{y}})$
\STATE $\mathbf{\boldsymbol{\delta}}_{\mathbf{y}}=\epsilon_{\mathbf{y}} \cdot \operatorname{sign}(\mathbf{\nabla}_{\mathbf{y}} \mathcal{L}(f(\mathbf{x}_{i} +\mathbf{\boldsymbol{\eta}}; \mathbf{w}), \mathbf{y}_{i}))$
\STATE $\mathbf{\boldsymbol{\delta}}_{\mathbf{y}}=\Pi_{[0, \epsilon_{\mathbf{y}}]}[\mathbf{\boldsymbol{\delta}}_{\mathbf{y}} + \mathbf{\boldsymbol{\eta}}_{\mathbf{y}}]$
\STATE $\mathcal{D}^{\boldsymbol{\delta}}_{i}= \mathbf{\boldsymbol{\delta}}$
\STATE $ \mathbf{w} \leftarrow \mathbf{w} -\mathbf{\nabla}_{\mathbf{w}}\mathcal{L}(f(\mathbf{x}_{i} + \mathbf{\boldsymbol{\delta}}; \mathbf{w}), \textrm{norm}(\mathbf{y}_{i}+\mathbf{\boldsymbol{\delta}}_{\mathbf{y}})) $
\ELSE
\STATE $\mathbf{\boldsymbol{\eta}} =\mathcal{D}^{\boldsymbol{\delta}}_{i} $
\STATE $\mathbf{g}_{c} =\operatorname{sign}\left(\nabla_{\mathbf{x}_i} \mathcal{L}(f(\mathbf{x}_i+\boldsymbol{\eta} ; \mathbf{w}), \mathbf{y}_{i})\right)$
\STATE $\mathcal{D}^{m}_{i}= \mu \cdot \mathcal{D}^{m}_{i} + g_{c}$
\STATE $ \boldsymbol{\delta} =\Pi_{[-\epsilon, \epsilon]} [ \boldsymbol{\eta}+ \alpha  \cdot \mathbf{g}_{c} ]$
\STATE $\mathcal{D}^{\boldsymbol{\delta}}_{i} =\Pi_{[-\epsilon, \epsilon]} [ \boldsymbol{\eta}+ \alpha  \cdot  \operatorname{sign} (\mathcal{D}^{m}_{i}) ]$
\STATE $\mathbf{y}_{i}=\textrm{norm}(\mathbf{y}_{i}+\mathbf{\boldsymbol{\eta}}_{\mathbf{y}})$
\STATE $\mathbf{\boldsymbol{\delta}}_{\mathbf{y}}=\epsilon_{\mathbf{y}} \cdot \operatorname{sign}(\mathbf{\nabla}_{\mathbf{y}} \mathcal{L}(f(\mathbf{x}_{i} +\mathbf{\boldsymbol{\eta}}; \mathbf{w}), \mathbf{y}_{i}))$
\STATE $\mathbf{\boldsymbol{\delta}}_{\mathbf{y}}=\Pi_{[0, \epsilon_{\mathbf{y}}]}[\mathbf{\boldsymbol{\delta}}_{\mathbf{y}} + \mathbf{\boldsymbol{\eta}}_{\mathbf{y}}]$
\STATE $ \mathbf{w} \leftarrow \mathbf{w} -\nabla_{\mathbf{w}}\mathcal{L}(f(\mathbf{x}_{i} + \boldsymbol{\delta}; \mathbf{w}), \textrm{norm}(\mathbf{y}_{i}+\boldsymbol{\delta}_{\mathbf{y}})) $
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> algo/FGSM_MEP.tex <==
\begin{algorithm}[t]
\caption{FGSM-MEP}
\label{alg:FGSM_MEP}
\begin{algorithmic}[1]
\REQUIRE
The epoch $N$, the maximal perturbation $\epsilon$, the maximal label perturbation $\epsilon_{\mathbf{y}}$, the step size $\alpha$, the dataset $\mathcal{D}$ including the benign sample $\mathbf{x}$ and the label $\mathbf{y}$, the dataset size $M$, the network $f(\cdot, \mathbf{w})$ with parameters $\mathbf{w}$, the decay factor $\mu$, the hyper-parameter $\lambda$, the adversarial initialization set $\mathcal{D}^{\mathbf{\boldsymbol{\delta}}}$ and the historical model gradient $\mathcal{D}^{m}$.
%The watermark image $W$, the host image $H$, the well-trained classifier $f$

\FOR{$n=1,...,N$}
\FOR{$i=1,...,M$}
\IF{$n==1$}
\STATE $\boldsymbol{\delta}_{pgi} =\mathbf{U}(-\epsilon ,\epsilon) $
\STATE $\mathbf{g}_{c} =\operatorname{sign}\left(\nabla_{\mathbf{x}_i} \mathcal{L}(f(\mathbf{x}_i+\boldsymbol{\delta}_{pgi} ; \mathbf{w}), \mathbf{y}_i)\right)$
\STATE $\mathcal{D}^{m}_{i}= \mathbf{g}_{c}$
\STATE $ \mathbf{\boldsymbol{\delta}_{adv}} =\Pi_{[-\epsilon, \epsilon]} [ \boldsymbol{\delta}_{pgi}+ \alpha \cdot \mathbf{g}_{c} ]$
\STATE $\mathcal{D}^{\boldsymbol{\delta}}_{i}= \boldsymbol{\delta}_{adv}$
\STATE $ \mathbf{w} \leftarrow \mathbf{w} -\mathbf{\nabla}_{\mathbf{w}}[\mathcal{L}(f(\mathbf{x}_{i} + \boldsymbol{\delta}_{adv}; \mathbf{w}), \mathbf{y}_i) +
\lambda \cdot\left\|f(\mathbf{x}+\boldsymbol{\delta}_{adv} ; \mathbf{w})-{f}(\mathbf{x}+\boldsymbol{\delta}_{pgi}; \mathbf{w})\right\|_{2}^{2}] $
\ELSE
\STATE $\boldsymbol{\delta}_{pgi} =\mathcal{D}^{\boldsymbol{\delta}}_{i} $
\STATE $\mathbf{g}_{c} =\operatorname{sign}\left(\nabla_{\mathbf{x}_i} \mathcal{L}(f(\mathbf{x}_i+\boldsymbol{\delta}_{pgi} ; \mathbf{w}), \mathbf{y}_{i})\right)$
\STATE $\mathcal{D}^{m}_{i}= \mu \cdot \mathcal{D}^{m}_{i} + \mathbf{g}_{c}$
\STATE $ \boldsymbol{\delta}_{adv} =\Pi_{[-\epsilon, \epsilon]} [ \boldsymbol{\delta}_{pgi}+ \alpha  \cdot \mathbf{g}_{c} ]$
\STATE $\mathcal{D}^{\boldsymbol{\delta}}_{i} =\Pi_{[-\epsilon, \epsilon]} [ \boldsymbol{\delta}_{pgi}+ \alpha  \cdot  \operatorname{sign} (\mathcal{D}^{m}_{i}) ]$
\STATE $ \mathbf{w} \leftarrow \mathbf{w} -\mathbf{\nabla}_{\mathbf{w}}[\mathcal{L}(f(\mathbf{x}_{i} + \mathbf{\boldsymbol{\delta}}_{adv}; \mathbf{w}), \mathbf{y}_i) +
\lambda \cdot\left\|f(\mathbf{x}+\boldsymbol{\delta}_{adv} ; \mathbf{w})-{f}(\mathbf{x}+\boldsymbol{\delta}_{pgi}; \mathbf{w})\right\|_{2}^{2}] $
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> fig/Ablation.tex <==
\begin{figure}[t]

        \centering
        \includegraphics[width=0.65\linewidth]{image/comparsion_regularizer.pdf}
        \label{fig:Ablation_Study}
        \vspace{-3mm}
  \caption{Ablation study of our proposed regularization using ResNet18 on the CIFAR-10 database. x-axis represents the attack method. y-axis represents robust accuracy.}
\label{fig:Ablation}
\end{figure}

==> fig/FGSM_MEP_test.tex <==
\begin{figure}[t]
\begin{subfigure}[t]{1\linewidth} 
        \centering
        \includegraphics[width=0.75\linewidth]{image/FGSM_MEP_test.png}
        \label{fig:difference_a}
    \end{subfigure} 

\vspace{-3mm}
  \caption{The PGD-10 accuracy of the proposed methods on the CIFAR10 test database. }
\label{fig:FGSM_MEP_test}
\vspace{-3mm}
\end{figure}

==> fig/Free_VS_Random.tex <==
\begin{figure}
\begin{center}
 \includegraphics[width=0.9\linewidth]{image/Free_VS_Random.pdf}
\end{center}
\vspace{-5mm}
\caption{Attack success rate of random initialization and free initialization during the training process. }
\label{fig:Free_VS_Random}

\end{figure}

==> fig/HP.tex <==
\begin{figure}[htb]
\centering

\begin{minipage}[t]{0.45\linewidth}
\centering
\includegraphics[width=1\linewidth]{image/HP_delay.pdf}
%\caption{fig1}
\end{minipage}
\begin{minipage}[t]{0.45\linewidth}
\centering
\includegraphics[width=1\linewidth]{image/HP_lamda.pdf}
%\caption{fig2}
\end{minipage}%
%
\centering
\caption{\textbf{Ablation studies in $p$.} Measure performance in terms of attack success rate (\%). The value of $\alpha$ is fixed at 1, and the value of $\beta$ is fixed at 0.5. The adversarial examples are generated on PointNet.}
\label{fig:p}
\vspace{-5mm}
\end{figure}

==> fig/Label.tex <==
\begin{figure}[t]
 \begin{minipage}[c]{0.23\textwidth}
        \begin{subfigure}{\textwidth}
          \centering
          \includegraphics[width=\linewidth]{image/Lable_one_hot.png}
          \vspace{-1.7em}
          \caption{Ground Truth}
          \label{One-Hot Label}
        \end{subfigure}\\
        \begin{subfigure}{\textwidth}
          \centering
          \includegraphics[width=\linewidth]{image/Lable_LS.png}
          \vspace{-1.7em}
          \caption{Label Smoothing}
          \label{Model Prediction Label}
        \end{subfigure}%
\end{minipage}
\hspace{0.1cm}
 \begin{minipage}[c]{0.23\textwidth}
        \begin{subfigure}{\textwidth}
          \centering
          \includegraphics[width=\linewidth]{image/Lable_model_output.png}
          \vspace{-1.7em}
          \caption{Prediction on AEs}
           \label{Label Smoothing}
        \end{subfigure}\\
        \begin{subfigure}{\textwidth}
          \centering
          \includegraphics[width=\linewidth]{image/Lable_AL.png}
          \vspace{-1.7em}
          \caption{Ours}
          \label{Ours}
        \end{subfigure}%
\end{minipage}




\vspace{-3mm}
  \caption{ Distributions of different label methods on the CIFAR-10 dataset. The true category is `3’. $x$-axis represents the class index of CIFAR10 and $y$-axis represents the score of each class. (a) Original one-hot label. (b) Prediction Label on AEs. (c) Soft label generated by LS \cite{DBLP:conf/cvpr/SzegedyVISW16}. (d) Soft label generated by our method. Our method modify the ground truth lable to \textbf{keep away from} the prediction on AEs while LS does not consider this.  }
\label{fig:Lable}
\vspace{-3mm}
\end{figure}

==> fig/Label_v2.tex <==
\begin{figure}[t]
\begin{center}
 \includegraphics[width=1.0\linewidth]{image/Lable.pdf}
\end{center}
\vspace{-3mm}
  \caption{ Difference between label smoothing and our adversarial label perturbation on the CIFAR10 database.
%   Distributions of different label methods on the CIFAR-10 dataset. 
  The true category is `3’. $x$-axis represents the class index of CIFAR10 and $y$-axis represents the score of each class. (a) Ground Truth label. (b) Prediction on AEs. (c) Soft label generated by LS \cite{DBLP:conf/cvpr/SzegedyVISW16}. (d) Soft label generated by our method. 
  Our method decreases the probability of the true class while increases the probabilities of the other classes to varying degrees to \textbf{keep away from} the prediction on AEs while LS does not consider this.  
  }
\label{fig:Lable}
\vspace{-3mm}
\end{figure}

==> fig/diff.tex <==
\begin{figure}
\begin{center}
 \includegraphics[width=0.6\linewidth]{image/diff.pdf}
\end{center}
\caption{ Attack success rate of FGSM-RS, PGD-AT, FGSM-FI and FGSM-FIAL during the training process.}
\label{fig:diff}
\end{figure}

==> fig/fig_label_perturbation.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.46\linewidth} 
        \centering
        \includegraphics[width=1\linewidth]{image/fig_example_perturbation.pdf}
        \caption{Example perturbation}
        \label{fig:examp_perturb}
    \end{subfigure} 
    \hspace{5mm}
\begin{subfigure}[t]{0.46\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{image/fig_label_perturbation.pdf}
        \caption{Label perturbation}
        \label{fig:lb_perturb}
    \end{subfigure} 

\vspace{-3mm}
  \caption{Adversarial example perturbation and adversarial label perturbation in the \textbf{label} space.  The adversarial label is made away from the predicted label of AE.   }
\label{fig:label_perturb}
\vspace{-3mm}
\end{figure}

==> fig/framework.tex <==
\begin{figure*}
\begin{center}
 \includegraphics[width=0.85\linewidth]{image/framework.pdf}
\end{center}
\caption{ The framework of the proposed method. We propose free initialization and adversarial label to improve the fast adversarial training.}
\label{fig:framework}

\end{figure*}

==> fig/home.tex <==
\begin{figure}
\begin{center}
 \includegraphics[width=1.0\linewidth]{image/home.pdf}
\end{center}
\caption{ The Overview of the proposed FGSM-FIAL. We propose free initialization and adversarial label to improve the fast adversarial training.}
\label{fig:home}

\end{figure}

==> fig/label_v3.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.22\linewidth} 
        \centering
        \includegraphics[width=1\linewidth]{image/one-hot.pdf}
        \caption{Ground truth one-hot label}
        \label{fig:GT}
    \end{subfigure} 
    \hspace{2mm}
\begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{image/label_AEs.pdf}
        \caption{Prediction of AE}
        \label{fig:ae_prediction}
    \end{subfigure} 
% \hspace{2mm}
% \begin{subfigure}[t]{0.18\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth]{image/sign_label.pdf}
%         \caption{Scaled signed adversarial label perturbation}
%         \label{fig:lb_p}
%     \end{subfigure} 
\hspace{2mm}
\begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{image/ours.pdf}
        \caption{Adversarial label}
        \label{fig:adv_lb}
    \end{subfigure} 
\hspace{2mm}
\begin{subfigure}[t]{0.22\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{image/LS.pdf}
        \caption{Label smoothing}
        \label{fig:lb_smooth}
    \end{subfigure} 
\vspace{-3mm}
%   \caption{The generation of adversarial label perturbation. Similar to the generation of adversarial example, we can obtain the scaled sign adversarial label perturbation by using FGSM.   }
 \caption{The generation of adversarial label perturbation. 
 Similar to the generation of adversarial example, we can obtain adversarial label by using FGSM. 
 The generated adversarial label is made to stay way from the prediction of AE in the label space. 
 Adversarial label perturbation decreases the probability of the ground truth (GT) class and suppresses the probabilities of classes that are relative large in the prediction of AE (\emph{e.g.} class 0, 5, \emph{etc}. in (b)). 
 It guides the model to not confuse the GT class with those that have large probabilities, resulting in more robust model. 
While LS averagely increases the probabilities of the other classes and has no such guidance. 
%The adversarial label perturbation makes it more challenging for the model to fit the pair of AE and adversarial label than the pair of AE and  GT label, which helps achieve more smooth decision boundaries, resulting in more robust model.  
%Using the adversarial label to train model makes the trained model to output the prediction far away from these classes on AEs.  
}


\label{fig:label}
\vspace{-3mm}
\end{figure*}


==> fig/loss_land.tex <==
\begin{figure}
\begin{center}
 \includegraphics[width=0.75\linewidth]{image/loss_land.pdf}
\end{center}
\vspace{-3mm}
\caption{Adversarial example generation process of PGD-AT~\cite{madry2017towards}, FGSM-AT~ \cite{goodfellow2014explaining} FGSM-RS~\cite{shafahi2019adversarial}, and our FGSM-MEPAL in the loss landscape of binary classification. Background is the contour of cross entropy. The redder the color, the higher the loss. PGD-AT is a multi-step AT method that computes gradients w.r.t the input at each step. FGSM-AT is a single step AT method.
FGSM-RS uses a random initialization followed by FGSM, 
while our FGSM-MEPAL adopts an adversarial initialization formed by historically generated adversarial examples followed by FGSM. 
The last three methods compute gradients only once. 
}
\label{fig:contour_of_CE}
\vspace{-3mm}
\end{figure}

==> fig/overfitting.tex <==
\begin{figure}
\begin{center}
 \includegraphics[width=1\linewidth]{image/overfitting.pdf}
\end{center}
\caption{The PGD-10 accuracy of AT methods on the CIFAR10 database in the training phase. (a) The PGD-10 accuracy on the training dataset. (b) The PGD-10 accuracy on the test dataset. }
\label{fig:ovrrfitting}

\end{figure}

==> fig/overfitting_V2.tex <==
\begin{figure}[t]
\begin{subfigure}[t]{1\linewidth} 
        \centering
        \includegraphics[width=0.75\linewidth]{image/FGSM_AT_overfitting_train_V2.png}
        \caption{}
        \label{fig:difference_a}
    \end{subfigure} 
\begin{subfigure}[t]{1\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{image/FGSM_AT_overfitting_test_V2.png}
        \caption{}
        \label{fig:difference_b}
    \end{subfigure} 

\vspace{-3mm}
  \caption{The PGD-10 accuracy of AT methods on the CIFAR10 database in the training phase. (a) The PGD-10 accuracy on the training dataset. (b) The PGD-10 accuracy on the test dataset. }
\label{fig:ovrrfitting_V2}
\vspace{-3mm}
\end{figure}

==> latex/Analysis.tex <==
\section{Conclusion  and Discussion}
This work proposes a fast adversarial training method to overcome catastrophic overfitting and improve adversarial robustness by introducing the priori-guided adversarial initialization and the novel adversarial label perturbation. 
Specifically, after exploring three adversarial initialization strategies, we propose to use the momentum of adversarial gradients of all previous epochs as the initialization of FGSM for AE generation. 
Inspired by AE perturbation, we propose the adversarial label perturbation by adding adversarial perturbation to the ground truth label. 
The perturbed labels and AEs are used for training.
Evaluations on four databases demonstrate that the proposed method can prevent catastrophic overfitting and improve adversarial robustness without additional calculation cost. 

\noindent \textbf{Limitations.} 
Our method has a side effect of improving robustness, \textit{i.e.,} the clean accuracy decreases. 
This effect also exists in other FAT methods. 
It might limit the application of FAT. 
We will rethink the robustness and accuracy trade-off in the future. 

% A new AT mechanism is an urgent demand
% The trade-off between robust accuracy and clean accuracy has not been solved in this paper.
% This is a common problem and will be further studied in the future.



==> latex/proof.tex <==
\begin{proof}
    The first part of the desired result \eqref{eq:propo_1} is true by the Jensen's inequality as 
    \begin{equation}
        \left(\mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}\sim\boldsymbol{\Omega}}\Big[\big\|\boldsymbol{\hat{\delta}}_{adv}\big\|_2\Big]\right)^2\leq\mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}\sim\boldsymbol{\Omega}}\Big[\big\|\boldsymbol{\hat{\delta}}_{adv}\big\|^2_2\Big].
    \end{equation}
    In the following we focus on $\mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}\sim\boldsymbol{\Omega}}\Big[\|\boldsymbol{\hat{\delta}}_{adv}\|^2_2\Big]$. Denote
    \begin{equation}
        \boldsymbol{\nabla} = \nabla_{\mathbf{x}} \mathcal{L}(f(\mathbf{x}+\mathbf{\boldsymbol{\delta}_{pgi}}; \mathbf{w}), \mathbf{y}),
    \end{equation}
    we have
    \begin{equation}
        \label{eq:1}
        \begin{aligned}
            & & &\ \ \mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}\sim\boldsymbol{\Omega}}\Big[\|\boldsymbol{\hat{\delta}}_{adv}\|^2_2\Big]\\[5pt]
            & &=&\ \ \mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}}\Big[\big\|\Pi_{\boldsymbol{\Omega}}\big[\mathbf{\boldsymbol{\delta}_{pgi}}+\alpha\cdot\operatorname{sign}(\boldsymbol{\nabla})\big]\big\|^2_2\Big]\\[5pt]
            & &=&\ \ \sum_{i=1}^d \mathbb{E}_{\delta_{pgi}(i)}\Big[\Pi_{\boldsymbol{\Omega}}\big[\mathbf{\delta}_{pgi}(i)+\alpha\cdot\operatorname{sign}(\nabla_i)\big]^2\Big]\\[5pt]
            % & &=&\ \ d\cdot\mathbb{E}_{\delta_t(i)}\Big[\textbf{min}\Big\{|\delta_{t+1}(i)-\delta_{t}(i)|,\big|\mathbf{\delta}_t(i)+\alpha\cdot\operatorname{sign}(\nabla_i)\big|\Big\}^2\Big]\\[5pt]
            % & &=&\ \ d\cdot\mathbb{E}_{\delta_t(i)}\Big[\textbf{min}\Big\{|\delta_{t+1}(i)-\delta_{t}(i)|^2,\big(\mathbf{\delta}_t(i)+\alpha\cdot\operatorname{sign}(\nabla_i)\big)^2\Big\}\Big]\\[5pt]
            & &\leq&\ \ d\cdot\mathbb{E}_{\delta_{pgi}(i)}\Big[\textbf{min}\Big\{\frac{\epsilon^2}{d},\big(\mathbf{\delta}_{pgi}(i)+\alpha\cdot\operatorname{sign}(\nabla_i)\big)^2\Big\}\Big]\\[5pt]
            & &=&\ \ d\cdot\mathbb{E}_{r_i}\Bigg[\mathbb{E}_{\delta_{pgi}(i)}\Big[\textbf{min}\Big\{\frac{\epsilon^2}{d},\big(\mathbf{\delta}_{pgi}(i)+\alpha\cdot\operatorname{sign}(\nabla_i)\big)^2\Big\}\Big]\ \Bigg|\ \operatorname{sign}(\nabla_i)=r_i\Bigg],
        \end{aligned}
    \end{equation}
    where the last setp follows the low of total expectation as $r_i:=\operatorname{sign}(\nabla_i)$ is also a random variable depending on $\delta_t(i)$. 

    As $r_i$ is a binary random variable, we seperate the precodure into the following two cases:
    \begin{itemize}
        \item[(i)] $r_i=1$, the inner conditional expectation has the form:
        \begin{equation}
            \label{eq:2}
            \begin{aligned}
                & & &\ \ \int_{-\epsilon}^{\epsilon}\textbf{min}\left\{\frac{\epsilon^2}{d},(\delta_{pgi}(i)+\alpha)^2\right\}\frac{1}{2\epsilon}d\delta_{pgi}(i)\\[5pt]
                & &=&\ \ \frac{1}{2\epsilon}\int_{-\epsilon+\alpha}^{\epsilon+\alpha}\textbf{min}\left\{\frac{\epsilon^2}{d},x^2\right\}dx\\[5pt]
                & &=&\ \ \frac{1}{2\epsilon}\left(\int_{\epsilon d^{-1/2}}^{\epsilon+\alpha}\frac{\epsilon^2}{d}dx+\int_{-\epsilon+\alpha}^{\epsilon d^{-1/2}}x^2dx\right)\\[5pt]
                % & &=&\ \ \frac{\alpha^2}{2}+\frac{\epsilon^2}{3}-\frac{\alpha^3}{6\epsilon}.
                & &=&\ \ \frac{\epsilon}{2d}\left(\alpha+\epsilon-\epsilon d^{-1/2}\right)+\frac{1}{6\epsilon}\left(\epsilon^3d^{3/2}-(\alpha-\epsilon)^3\right)\\[5pt]
                & &=&\ \
                \frac{\epsilon(\alpha+\epsilon)}{2d}-
                \frac{\epsilon^2}{3d^{3/2}} -\frac{(\alpha-\epsilon)^3}{6\epsilon}\\[5pt]
                % \frac{\epsilon^2}{4d}+\frac{\alpha\epsilon}{4d}+\frac{\epsilon^2}{48}-\frac{1}{6\epsilon}(\alpha-\epsilon)^3\\[5pt].
                % & &\leq&\ \ \frac{\epsilon^2}{2d} - \frac{\epsilon^2}{3d^{3/2}}+\frac{\epsilon^2}{6}
                & &\leq&\ \ \frac{\epsilon^2}{d}.
            \end{aligned}
        \end{equation}
        \item[(ii)] $r_i=-1$, the inner conditional expectation will be:
        \begin{equation}
            \label{eq:3}
            \begin{aligned}
                & & &\ \ \int_{-\epsilon}^{\epsilon}\textbf{min}\left\{\frac{\epsilon^2}{d},(\delta_{pgi}(i)-\alpha)^2\right\}\frac{1}{2\epsilon}d\delta_t(i)\\[5pt]
                & &=&\ \ \frac{1}{2\epsilon}\int_{-\epsilon-\alpha}^{\epsilon-\alpha}\textbf{min}\left\{\frac{\epsilon^2}{d},x^2\right\}dx\\[5pt]
                & &=&\ \ \frac{1}{2\epsilon}\left(\int_{\epsilon d^{-1/2}}^{\epsilon-\alpha}x^2dx+\int_{-\epsilon-\alpha}^{\epsilon d^{-1/2}}\frac{\epsilon^2}{d}dx\right)\\[5pt]
                & &=&\ \ \frac{\epsilon}{2d}\left(\epsilon d^{-1/2}+\epsilon+\alpha\right)+\frac{1}{6\epsilon}\left((\epsilon-\alpha)^3-\epsilon^3d^{-3/2}\right)\\[5pt]
                & &=&\ \  \frac{\epsilon(\alpha+\epsilon)}{2d}+
                \frac{\epsilon^2}{3d^{3/2}} -\frac{(\alpha-\epsilon)^3}{6\epsilon}\\[5pt]
                % & &\leq                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &\ \  \frac{\epsilon^2}{d} + \frac{\epsilon^2}{2d^{3/2}} +  \frac{\epsilon^2}{6}
                & &\leq& \frac{\epsilon^2}{d} + \frac{2\epsilon^2}{3d^{3/2}}
                % & &\leq&\ \ \frac{\epsilon^2}{12}.        
            \end{aligned}
        \end{equation}
    \end{itemize}
    Combining \eqref{eq:2} and \eqref{eq:3} together with \eqref{eq:1}, we obtain
    \begin{equation*}
        \begin{aligned}
            & \mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}\sim\boldsymbol{\Omega}}\big[\|\boldsymbol{\hat{\delta}}_{adv}\|_2\big]&\leq&\ \ \sqrt{\ \mathbb{E}_{\boldsymbol{\hat{\delta}}_{adv}\sim\boldsymbol{\Omega}}\big[\|\boldsymbol{\hat{\delta}}_{adv}\|^2_2\big]}\\
            % & &\leq&\ \ \sqrt{\frac{3d^{1/2}+2+d^{3/2}}{6d}}\cdot\epsilon.
            & &\leq&\ \ \sqrt{1+\frac{2}{3\sqrt{d}}}\cdot\epsilon.
        \end{aligned}        
    \end{equation*}
\end{proof}
% \noindent\textbf{Remark.} By the monotonicity of the FGSM type methods \cite{dou2018mathematical}, we know that the bounded set $\boldsymbol{\Omega}$ will be shrinkage during the adversarial perturbation. It means that the proposed prior-guided adversarial initialization will conduct the more efficient step size than \cite{andriushchenko2020understanding}.

% \begin{equation}
%         \begin{aligned}
%               & & &\min_{\mathbf{w}} \mathbb{E}_{(\mathbf{x}, y) \sim \mathcal{D}}\left[\max_{\boldsymbol{\theta}}~\mathbb{E}_{ \mathbf{a} \sim p(\mathbf{a}| \mathbf{x};\boldsymbol{\theta})}~[\mathcal{L}_1(\mathbf{w},\boldsymbol{\theta})+ \alpha \mathcal{L}_2(\boldsymbol{\theta}) + \beta \mathcal{L}_3(\boldsymbol{\theta})]\right],
%         \end{aligned}
%         \label{eq:newAT_pro}
%     \end{equation}

==> table/LS.tex <==
\begin{table}[]

\centering

\scalebox{0.77}{

\begin{tabular}{c|c|c|c|c}
\toprule 
Method  & Clean          & PGD-50         & AA             & Time(min) \\ \midrule \midrule
FGSM-RS + LS ($\alpha$=0.1)   & 83.27          & 46.20          & 41.16          &   51   \\ %\hline
FGSM-RS + LS ($\alpha$=0.2)    & 84.32 & 46.58          & 42.95          &    51 \\
FGSM-MEP + LS ($\alpha$=0.1)   & 85.20          & 47.09          & 43.37          &   51  \\ %\hline
FGSM-MEP + LS ($\alpha$=0.2)    & \textbf{86.46} & 48.10          & 43.83          &    51  \\ %\hline
FGSM-MEPAL & 86.26          & \textbf{49.60} & \textbf{45.33} & 51     \\ \bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) using ResNet18 on the  CIFAR-10 dataset. 
% Number in bold indicates the best of the fast AT methods. 
}
\vspace{-3mm}
\label{table:LS}
\end{table}

==> table/Tiny_imagenet.tex <==
\begin{table}[t]


\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|c}
\hline
Tiny ImageNet              &      & Clean          & PGD-50         & AA             & Time(min)            \\ \hline
\multirow{2}{*}{PGD-AT}    & Best & 43.6           & 19.86          & 16.00          & \multirow{2}{*}{1833} \\ %\cline{2-5}
                           & Last & 45.28          & 15.4           & 12.84          &                      \\ \hline \hline
\multirow{2}{*}{FGSM-RS}   & Best & 44.98          & 17.36          & 14.08          & \multirow{2}{*}{339}  \\ %\cline{2-5}
                           & Last & 45.18          & 0.00           & 0.00           &                      \\ \hline
\multirow{2}{*}{FGSM-CKPT} & Best & \textbf{49.98} & 8.68           & 8.10           & \multirow{2}{*}{686}  \\ %\cline{2-5}
                           & Last & \textbf{49.98} & 8.68           & 8.10           &                      \\ \hline
\multirow{2}{*}{FGSM-GA}   & Best & 34.04          & 5.58           & 4.34           & \multirow{2}{*}{1054} \\ %\cline{2-5}
                           & Last & 34.04          & 5.58           & 4.34           &                      \\ \hline
\multirow{2}{*}{Free-AT(m=8)}   & Best & 38.9           & 11.02          & 9.28           & \multirow{2}{*}{1375} \\ %\cline{2-5}
                           & Last & 40.06          & 8.2            & 7.34           &                      \\ \hline
\multirow{2}{*}{FGSM-FI (ours)}   & Best & 45.46          & 19.08          & 15.32          & \multirow{2}{*}{339}  \\ %\cline{2-5}
                           & Last & 44.54          & 14.38          & 12.14          &                      \\ \hline
\multirow{2}{*}{FGSM-FIAL (ours)} & Best & 45.76          & \textbf{22.1}  & \textbf{16.14} & \multirow{2}{*}{339}  \\ %\cline{2-5}
                           & Last & 46.94          & \textbf{19.32} & \textbf{14.30} &                      \\ \hline
\end{tabular}
}
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the Tiny ImageNet database. Number in bold indicates the best of the fast AT methods. }
\label{table:Tiny_Imagnet}
\end{table}

==> table/cifar100.tex <==
\begin{table*}[t]
\centering


 \scalebox{0.9}{
\begin{tabular}{c|ccccccc|c}
\hline
CIFAR100                   &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{PGD-AT}    & Best & 57.52          & 29.60          & 28.99          & 28.87          & 28.85          & 25.48          & \multirow{2}{*}{284} \\ %\cline{2-8}
                           & Last & 57.50          & 29.54          & 29.00          & 28.90          & 27.60          & 25.48          &                      \\ \hline \hline
\multirow{2}{*}{FGSM-RS}   & Best & 49.85          & 22.47          & 22.01          & 21.82          & 20.55          & 18.29          & \multirow{2}{*}{70}  \\ %\cline{2-8}
                           & Last & 60.55          & 00.45          & 00.25          & 00.19          & 00.25          & 0.00           &                      \\ \hline
\multirow{2}{*}{FGSM-CKPT} & Best & \textbf{61.93} & 16.58          & 15.47          & 15.19          & 16.40          & 14.17          & \multirow{2}{*}{92}  \\ %\cline{2-8}
                           & Last & {61.93} & 16.58          & 15.47          & 15.19          & 16.40          & 14.17          &                      \\ \hline
\multirow{2}{*}{FGSM-GA}   & Best & 47.57          & 21.33          & 20.83          & 20.64          & 19.11          & 17.20          & \multirow{2}{*}{187} \\ %\cline{2-8}
                           & Last & 55.1           & 18.84          & 17.95          & 17.72          & 18.04          & 16.10          &                      \\ \hline
\multirow{2}{*}{Free-AT(m=8)}   & Best & 44.03          & 20.61          & 20.23          & 20.23          & 18.26          & 16.46          & \multirow{2}{*}{229} \\ %\cline{2-8}
                           & Last & 48.03          & 20.17          & 20.29          & 20.19          & 18.20          & 16.46          &                      \\ \hline
\multirow{2}{*}{FGSM-FI (ours)}   & Best & 60.18          & 25.97          & 25.02          & 24.78          & 24.82          & 21.72          & \multirow{2}{*}{70}  \\ %\cline{2-8}
                           & Last & 61.12          & 24.94          & 23.76          & 23.43          & 24.21          & 20.85          &                      \\ \hline
\multirow{2}{*}{FGSM-FIAL (ours)} & Best & 61.81          & \textbf{30.90}  & \textbf{29.91} & \textbf{29.61} & \textbf{25.76} & \textbf{23.75} & \multirow{2}{*}{70}  \\ %\cline{2-8}
                           & Last & \textbf{61.96}          & \textbf{30.47} & \textbf{29.59} & \textbf{29.35} & \textbf{25.73} & \textbf{23.60} &                      \\ \hline
\end{tabular}
}
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the CIFAR100 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar100_ResNet}
\end{table*}

==> table/cifar10_ResNet.tex <==
\begin{table*}[t]
\centering


 \scalebox{0.9}{
\begin{tabular}{c|ccccccc|c}
\hline
CIFAR10                    &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{PGD-AT}    & Best & 82.64          & 53.15          & 52.56          & 52.15          & 51.14          & 48.81          & \multirow{2}{*}{261} \\ %\cline{2-8}
                           & Last & 82.86          & 52.85          & 52.27          & 51.98          & 51.32          & 48.54          &                      \\ \hline \hline
\multirow{2}{*}{FGSM-RS}   & Best & 73.81          & 42.31          & 41.55          & 41.26          & 39.84          & 37.07          & \multirow{2}{*}{55}  \\ %\cline{2-8}
                           & Last & 83.82          & 00.09          & 00.04          & 00.02          & 0.00           & 0.00           &                      \\ \hline
\multirow{2}{*}{FGSM-CKPT} & Best & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 37.15          & \multirow{2}{*}{83}  \\ %\cline{2-8}
                           & Last & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 37.15          &                      \\ \hline
\multirow{2}{*}{FGSM-GA}   & Best & 83.96          & 49.23          & 47.57          & 46.89          & 47.46          & 43.45          & \multirow{2}{*}{178} \\ %\cline{2-8}
                           & Last & 84.43          & 48.67          & 46.66          & 46.08          & 46.75          & 42.63          &                      \\ \hline
\multirow{2}{*}{Free-AT(m=8)}   & Best & 74.87          & 43.7           & 42.84          & 42.6           & 41.09          & 39.11          & \multirow{2}{*}{215} \\ %\cline{2-8}
                           & Last & 74.87          & 43.58          & 42.81          & 42.62          & 41.1           & 39.05          &                      \\ \hline
\multirow{2}{*}{FGSM-FI (ours)}   & Best & 85.97          & 48.2           & 46.73          & 46.23          & 46.85          & 43.39          & \multirow{2}{*}{55}  \\ %\cline{2-8}
                           & Last & 86.3           & 47.38          & 45.83          & 45.27          & 46.14          & 42.84          &                      \\ \hline
\multirow{2}{*}{FGSM-FIAL (ours)} & Best & 86.26          & \textbf{51.51} & \textbf{49.98} & \textbf{49.60}  & \textbf{47.98} & \textbf{45.33} & \multirow{2}{*}{55}  \\ %\cline{2-8}
                           & Last & 86.72          & \textbf{50.56} & \textbf{48.72} & \textbf{48.09} & \textbf{46.97} & \textbf{44.09} &                      \\ \hline
\end{tabular}
}
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar10_ResNet}
\end{table*}

==> table/cifar10_v2.tex <==
\begin{table*}[t]
\centering


\scalebox{1}{
\begin{tabular}{c|ccccccc|c}
\hline
CIFAR10                    &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & Time(min)            \\ \hline
\multirow{2}{*}{PGD-AT}    & Best & 82.64          & 53.15          & 52.56          & 52.15          & 51.14          & 48.81          & \multirow{2}{*}{261} \\ %\cline{2-8}
                           & Last & 82.86          & 52.85          & 52.27          & 51.98          & 51.32          & 48.54          &                      \\ \hline \hline
\multirow{2}{*}{FGSM-RS}   & Best & 73.81          & 42.31          & 41.55          & 41.26          & 39.84          & 37.07          & \multirow{2}{*}{55}  \\ %\cline{2-8}
                           & Last & 83.82          & 00.09          & 00.04          & 00.02          & 0.00           & 0.00           &                      \\ \hline
\multirow{2}{*}{FGSM-CKPT} & Best & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 37.15          & \multirow{2}{*}{83}  \\ %\cline{2-8}
                           & Last & \textbf{88.29} & 42.05          & 39.80          & 39.11          & 41.46          & 37.15          &                      \\ \hline
\multirow{2}{*}{FGSM-GA}   & Best & 83.96          & 49.23          & 47.57          & 46.89          & 47.46          & 43.45          & \multirow{2}{*}{178} \\ %\cline{2-8}
                           & Last & 84.43          & 48.67          & 46.66          & 46.08          & 46.75          & 42.63          &                      \\ \hline
\multirow{2}{*}{Free-AT(m=8)}   & Best & 74.87          & 43.7           & 42.84          & 42.6           & 41.09          & 39.11          & \multirow{2}{*}{215} \\ %\cline{2-8}
                           & Last & 74.87          & 43.58          & 42.81          & 42.62          & 41.1           & 39.05          &                      \\ \hline
\multirow{2}{*}{FGSM-FI (ours)}   & Best & 85.97          & 48.2           & 46.73          & 46.23          & 46.85          & 43.39          & \multirow{2}{*}{55}  \\ %\cline{2-8}
                           & Last & 86.3           & 47.38          & 45.83          & 45.27          & 46.14          & 42.84          &                      \\ \hline
\multirow{2}{*}{FGSM-FIAL (ours)} & Best & 86.26          & \textbf{51.51} & \textbf{49.98} & \textbf{49.60}  & \textbf{47.98} & \textbf{45.33} & \multirow{2}{*}{55}  \\ %\cline{2-8}
                           & Last & 86.72          & \textbf{50.56} & \textbf{48.72} & \textbf{48.09} & \textbf{46.97} & \textbf{44.09} &                      \\ \hline
\end{tabular}
}
\caption{Comparisons of clean and robust accuracy (\%) and training time (minute) on the CIFAR10 database. Number in bold indicates the best of the fast AT methods. }
\label{table:cifar10_ResNet}
\end{table*}
